UniSRM: A Unified Speech Reward Model for Reasoning-Based Fine-grained Assessment

Evaluating speech generation still relies heavily on human judgments, such as Mean Opinion Score (MOS), which are expensive, subjective, and difficult to reproduce at scale. While a few recent studies have begun to explore AudioLLM-based judge models, existing efforts typically target only a narrow set of scenarios (e.g., utterance-level quality or single-turn dialogue) and provide limited coverage of diverse speech generation tasks and evaluation dimensions. In this work, we propose UniSRM, a unified speech reward model that can support multi-dimensional, interpretable reward signals with reliable reasoning. To support training and evaluation, we introduce UniSRM-Data and UniSRM-Bench, covering speech evaluation tasks from utterance-level quality to context-level coherence. Based on this dataset, we present the unified speech reward model, UniSRM, with a two-stage pipeline that enables reasoning-based fine-grained assessment. Furthermore, we introduce Reasoning-Consistent Rewards to improve the reliability of the reasoning process. Experiments show that UniSRM delivers more reliable and human-aligned judgments across a broad range of speech evaluation tasks, offering a practical foundation for scalable and unified evaluation of speech quality.

==> tables/task3_zh_abla.tex <==
 
\begin{table*}[tb]
\centering
\setlength{\tabcolsep}{1.0mm}
\begin{tabular}{ccccc}
\toprule
\multirow{1}{*}{\textbf{Model}}            &
\multirow{1}{*}{\textbf{Text}} &
\multirow{1}{*}{\textbf{Scenario}} &
\multirow{1}{*}{\textbf{Naturalness}} &
\multirow{1}{*}{\textbf{Avg}}
\\  \midrule

UniSRM(Ours) & 86.76&	91.11&	88.14&	88.67\\
$w/o$ RCR-GRPO & 84.78&	81.03&	78.66&	81.49\\
$w/o$ GRPO & 85.38&	70.75&	68.97&	75.03\\

\bottomrule
\end{tabular}
\caption{Multi-dimensional results on the Chinese split of scenario-aware speech preference task. Results are reported as accuracy ($\uparrow$, \%).}
\label{exp_task2_zh_abla}
\end{table*}
